Manipulation Testing in Boundary Discontinuity Designs

We propose the first manipulation test designed for boundary discontinuity designs (BDDs) with general boundary shapes. A BDD is a multidimensional extension of the regression discontinuity design (RDD) in which treatment assignment is determined by whether the multidimensional running variable crosses a lower-dimensional boundary set. The test avoids multivariate density estimation and builds on the observation that, in the absence of manipulation, observations near the boundary should be approximately evenly split between treatment and control within arbitrary groups defined by their projections onto the boundary. We test this implication using a collection of binomial balance tests on observations near the boundary, with groups formed by k-means clustering. We establish the asymptotic validity of the test under suitable regularity conditions. We also evaluate finite-sample performance through Monte Carlo simulations and illustrate the test in three empirical applications.

==> tables/empirical_tests.tex <==
\begin{table}[htbp]
\centering
\caption{\small Simulation-based $p$-values ($\hat{p}$) for the BDD manipulation test at level $\alpha = 0.05$, for $q \in \{100, 150, 200, n^{0.6}\}$ (with $n^{0.6}$ rounded to the nearest integer and application-specific $n$) and cluster-count grids $\mathcal{K} \in \bigl\{\{1\},\{1,\ldots,50\},\{1,\ldots,5\},\{1,5,10,15,20\}\bigr\}$. Each cell reports the simulation-based $p$-value $\hat{p}$; --- indicates infeasible pairs with $\max(\mathcal{K}) > q$.}
\label{tab:tests}
\vspace{0.3cm}
\input{tables/subtable_frey.tex}
\vspace{0.4cm}
\input{tables/subtable_keele_titiunik.tex}
\vspace{0.4cm}
\input{tables/subtable_elacqua.tex}
\end{table}


==> tables/subtable_elacqua.tex <==
\begin{minipage}{0.92\textwidth}
    \centering
    {\footnotesize
    \begin{tabular}{lcccc}
    \hline \hline
     \multicolumn{5}{c}{\cite{elacqua2024effects}} \\
     \multicolumn{5}{c}{$n = 2{,}039$} \\
    \hline
    $\mathcal{K}$ $\backslash$ $q$ & 97 & 100 & 150 & 200 \\
    \hline 
    $\{1\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,\ldots,50\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,\ldots,5\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,5,10,15,20\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline \hline 
    \end{tabular}
    }
\end{minipage}


==> tables/subtable_frey.tex <==
\begin{minipage}{0.92\textwidth}
    \centering
    {\footnotesize
    \begin{tabular}{lcccc}
    \hline \hline
     \multicolumn{5}{c}{\cite{frey:2019}} \\
     \multicolumn{5}{c}{$n = 2{,}045$} \\
    \hline
    $\mathcal{K}$ $\backslash$ $q$ & 97 & 100 & 150 & 200 \\
    \hline 
    $\{1\}$ & 0.682 & 0.479 & 0.804 & 0.625 \\
    $\{1,\ldots,50\}$ & 0.279 & 0.258 & 0.465 & 0.346 \\
    $\{1,\ldots,5\}$ & 0.118 & 0.139 & 0.740 & 0.827 \\
    $\{1,5,10,15,20\}$ & 0.319 & 0.364 & 0.447 & 0.641 \\
    \hline \hline 
    \end{tabular}
    }
\end{minipage}


==> tables/subtable_keele_titiunik.tex <==
\begin{minipage}{0.92\textwidth}
    \centering
    {\footnotesize
    \begin{tabular}{lcccc}
    \hline \hline
     \multicolumn{5}{c}{\cite{keele/titiunik:2015}} \\
     \multicolumn{5}{c}{$n = 7{,}523$} \\
    \hline
    $\mathcal{K}$ $\backslash$ $q$ & 100 & 150 & 200 & 212 \\
    \hline 
    $\{1\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,\ldots,50\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,\ldots,5\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    $\{1,5,10,15,20\}$ & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline \hline 
    \end{tabular}
    }
\end{minipage}


==> tables/table_counterexample_mc.tex <==
\begin{table}[]
\centering
\caption{\small Empirical frequency of rejections of the one-dimensional manipulation test in \citet{cattaneo2018manipulation} at nominal level 0.05, for the design in \eqref{eq:counterexample}. $m = 1000$ Monte Carlo replications per~$n$.}
\vspace{0.5cm}
\label{tab:counterexample_mc}
\begin{tabular}{c@{\hspace{1.5em}}r}
\hline \hline
$n$ & Rejection rate \\
\hline
500 & 0.349 \\
1{,}000 & 0.632 \\
2{,}000 & 0.891 \\
5{,}000 & 0.998 \\
\hline
\hline \hline
\end{tabular}
\end{table}

